Safe and Stable Control Synthesis for Uncertain System Models via Distributionally Robust Optimization

This paper considers enforcing safety and stability of dynamical systems in the presence of model uncertainty. Safety and stability constraints may be specified using a control barrier function (CBF) and a control Lyapunov function (CLF), respectively. To take model uncertainty into account, robust and chance formulations of the constraints are commonly considered. However, this requires known error bounds or a known distribution for the model uncertainty, and the resulting formulations may suffer from over-conservatism or over-confidence. In this paper, we assume that only a finite set of model parametric uncertainty samples is available and formulate a distributionally robust chance-constrained program (DRCCP) for control synthesis with CBF safety and CLF stability guarantees. To facilitate efficient computation of control inputs during online execution, we present a reformulation of the DRCCP as a second-order cone program (SOCP). Our formulation is evaluated in an adaptive cruise control example in comparison to 1) a baseline CLF-CBF quadratic programming approach, 2) a robust approach that assumes known error bounds of the system uncertainty, and 3) a chance-constrained approach that assumes a known Gaussian Process distribution of the uncertainty.

==> computation-graph.tex <==
\begin{tikzpicture}
\providecommand{\bfx}{\mathbf{x}}
\providecommand{\Lie}{\mathcal{L}}
\providecommand{\grad}{\nabla}
\providecommand{\GP}{GP}
\providecommand{\ubfu}{\underline{\mathbf{u}}}
\node [] (gh) {$\grad_\bfx h(\bfx)$};

\node [right=of gh] (L1) {$\underbrace{\grad_\bfx h(\bfx)^\top f(\bfx)}_{\Lie_f h(\bfx)}$};

\path [->,color=red] (gh)  edge [above] node {$[\cdot]$} (L1);

\node [below=of L1] (f1) {$f(\bfx) \sim \GP $};

\path [->,color=red] (f1)  edge [left] node {$[\cdot]$} (L1);

\node [right=of L1] (gL1) {$\grad_\bfx \Lie_f h(\bfx)$};

\path [->,color=blue] (L1)  edge [above] node {$\grad_\bfx$} (gL1);

\node [right=of gL1] (L2) {$\grad_\bfx[\Lie_f h(\bfx)]^\top F(\bfx) \ubfu$};

\node [below=38pt of L2] (f2) {$F(\bfx)\ubfu \sim \GP $};

\path [->,color=red] 
(f2) edge 
    node[above] {$[\cdot]$}
    node[below] {$\ubfu = [1, \mathbf{0}^\top_m]^\top$} 
 (f1);

\path [->,color=red] (f2)  edge [left] node {$[\cdot]$} (L2);

\path [->,color=red] (gL1)  edge [above] node {$[\cdot]$} (L2);

%\node [right=of L2] (gL2) {};
%\draw[dotted] (L2) -- (gL2) ;
%\path[clip] (gh.north west) rectangle (f2.south east); 
\end{tikzpicture}



==> tex/Problem_formulation_another_uncertainty.tex <==
\section{Problem Formulation}
\label{sec: problem}

We study the problem of enforcing safety and stability for unknown system dynamics, using the newly-developed techniques and analysis in DRCCP. 



% \TODO{Main idea: by considering the wasserstein ball with radius $r$ around the empirical distribution of $\textit{CLC}(\bfx,\bfu), \textit{CBC}(\bfx,\bfu)$ with $r$ being tunable, we can enforce stability and safety of the dynamic system without knowing explicitly the error models in $F$ and/or $h$.}

\subsection{DRCCP Formulation For Continuous-time System}
Formally, we consider a uncertain non-linear control-affine system:
%
\begin{equation}\label{eq: uncertain_dynamic_1}
\begin{aligned}
    &\dot{\bfx} = f(\bfx)+ g(\bfx) \bfu \delequal F(\bfx)\ubfu =\\
    &(\tilde{F}(\bfx) + (p_1(\bfx)\xi_1 \oplus p_2(\bfx)\xi_2 \oplus \cdots \oplus p_{m+1}(\bfx)\xi_{m+1}))\ubfu
\end{aligned}
\end{equation}
%
where the admissible control input space is given by $\underline{\calU} \coloneqq \{\ubfu \in \mathbb{R}^{m+1} \,|\, \ubfu^\top \boldsymbol{e}_1 = 1\}$, where $\boldsymbol{e}_1 \in \mathbb{R}^{m+1}$ is the basis vector with $1$ at the first entry and $0$ elsewhere. We use $\tilde{F}$ to denote the estimated system dynamics. For $1 \leq i \leq m+1$, we use $p_i(\bfx) \in \mathbb{R}^{n \times p}$ and $\xi_i \in \mathbb{R}^p$ to denote the parametric uncertainty. We use $\oplus$ to denote appending a column vector to a matrix, meaning that $\bfA \oplus \bfb = [\bfA \; \bfb]$.

In the following, we write
%
\begin{equation*}
    \bfp(\bfx,\xi) = p_1(\bfx)\xi_1 \oplus p_2(\bfx)\xi_2 \oplus \cdots \oplus p_{m+1}(\bfx)\xi_{m+1}.
\end{equation*}
%
We also define 
%
\begin{equation}
\label{uncertainty_append}
    \bfxi \delequal \begin{bmatrix}
    \xi_1 \\
    \xi_2 \\
    \vdots \\
    \xi_{m+1}
    \end{bmatrix} \in \Xi \subseteq \mathbb{R}^{p(m+1)}
\end{equation}


% In the following discussion, we assume $\bfxi(\bfx) = \bfxi$ is constant over the state space. 

\begin{problem}[\textbf{Uncertainty Collection with State-Control Sequences}]\label{prob: uncertainty_collection}
For some unknown system dynamics $\dot{\bfx} = F(\bfx)\ubfu$, given a state-control dataset $\mathcal{D} = \{t_{0:N}^{(i)}, \bfx_{0:N}^{(i)}, \ubfu_{0:N}^{(i)}\}_{i=1}^{D}$ of state sequences $\bfx_{0:N}^{(i)}$ obtained by applying random control inputs $\bfu_{0:N}^{(i)}$ to the robot with initial condition $\bfx_{0}^{(i)}$, compute the approximated system dynamics $\tilde{F}$, the parametric matrix $p_i(\bfx)$, and the uncertainty observations $\{\bfxi_i\}_{i=1}^N$ for $\bfxi$. 
\end{problem}

\begin{problem}[\textbf{Safety and Stability For Uncertain Systems}]\label{prob: data_driven_safety_stability}
For some unknown system dynamics $F(\bfx)$, given the predicted system dynamics $\tilde{F}(\bfx)$ and a set of observations $\{\bfxi_i\}_{i=1}^N$ of the uncertainty $\bfxi$, design a feedback controller $\bfk$ with a risk-tolerance parameter $\epsilon$ such that, for each $\bfx \in \calX$: 
\begin{align}
    &\inf_{\mathbb{P} \in \calM_{N}^{r_1}}\mathbb{P}(\textit{CLC}(\bfx,\underline{\bfk}(\bfx), \bfxi)) \leq \delta ) \geq 1 - \epsilon \notag\\
    &\inf_{\mathbb{P} \in \calM_{N}^{r_2}}\mathbb{P}(\textit{CBC}(\bfx,\underline{\bfk}(\bfx), \bfxi)) \geq 0 ) \geq 1 - \epsilon,
\end{align}
where $\calM_{N}^{r_1}, \calM_{N}^{r_2}$ is the ambiguity set with user-specified wasserstein radius $r_1$ and $r_2$. 


% \TODO{Ideally, by applying distributional robust idea to the CLF-CBF-QP formulation, even though we are only given offline uncertainty measurements $\xi_i$, our controller is able to enforce stability and safety for out-of-distribution samples online (e.g. varying wind speeds for quadrotor, different frictions for ground robots, different loads for delivery robots).}

\end{problem}

==> tex/Related_work.tex <==
\section{Related Work}
\label{sec: related_work}
In this section, we review some previous work on safety and stability verification for uncertain systems. 
